Status and Perspectives of Neutrino Physics

This review demonstrates the unique role of the neutrino by discussing in detail the physics of and with neutrinos. We deal with neutrino sources, neutrino oscillations, absolute masses, interactions, the possible existence of sterile neutrinos, and theoretical implications. In addition, synergies of neutrino physics with other research fields are found, and requirements to continue successful neutrino physics in the future, in terms of technological developments and adequate infrastructures, are stressed.

==> WG1/WG1_theor.tex <==
\subsection{Theoretical implications of the PMNS matrix}
\label{WG1:Sect:PMNS-Theory}

\subsubsection{Introduction}
\label{WG1:SubSec:PMNS-Theory:Intro}

The peculiar pattern observed for the three PMNS mixing angles, with
$\theta_{12}$ and $\theta_{23}$ being large while $\theta_{13}$ is
small (but not tiny) is a strong contrast to the CKM matrix.
This poses intriguing questions on the origin of the leptonic flavor 
structure.
It remains an open question as to whether these mixing patterns
reflect some deeper theoretical principle such as a broken flavor
symmetry, or they are purely random or ``anarchic''.
The relationship, if any, between the PMNS and CKM matrices is also an
unknown.
These issues are a major concern in the literature
(see~\cite{King:2013eh,Xing:2019vks,Feruglio:2019ktm} for
comprehensive reviews of flavor symmetries and~\cite{deGouvea:2003xe}
for an analysis of the anarchy hypothesis). 

The nature of CP violating phases is a related theoretical challenge, with ramifications through leptogenesis for cosmology, as well as for particle physics \emph{per se}. The current indications for a Dirac phase in the vicinity of $-\pi/2$ (adopting the standard PMNS parameterisation) invite thoughts of flavor symmetries, while the existence or not of CP violating Majorana phases remains undetermined. Leptogenesis can proceed through any of these phases, or others that pertain to heavy neutral lepton partners of the light active neutrinos. Observation of low energy CP violation in the lepton sector, together with that of lepton number violation, would provide circumstantial evidence of leptogenesis as the origin of the observed baryon asymmetry of the Universe.

The PMNS matrix is exactly a $3 \times 3$ unitary matrix for two important neutrino mass scenarios: (1) the case of three Dirac neutrinos where their mass generation occurs in exactly the same way as for the charged fermions, in presence of lepton number conservation, and (2) the case of three left-handed Majorana neutrinos with no additional neutrino-like states playing any role in the mass generation, as is the case for the type II seesaw model~\cite{Magg:1980ut,Schechter:1980gr,Cheng:1980qt,Lazarides:1980nt,Wetterich:1981bx,Mohapatra:1980yp}. However, if there are additional neutrino-like states with Majorana masses, they generically couple with the three known neutrino flavors via a Yukawa interaction with the Higgs, unless a symmetry is invoked to forbid these terms. Once the Higgs acquires a vacuum expectation value, mixing arises and affects all the neutrino and neutrino-like states rendering the $3 \times 3$ PMNS matrix only approximately unitary. For instance, this is the case in the most studied type I see-saw models~\cite{Minkowski:1977sc,GellMann:1980vs,Yanagida:1979as,Glashow:1979nm,Mohapatra:1979ia}. If the scale of the see-saw mechanism is low, or in the presence of additional states, as in inverse~\cite{Wyler:1982dd,Mohapatra:1986aw,Mohapatra:1986bd}, linear~\cite{Akhmedov:1995vm,Barr:2003nn,Malinsky:2005bi} or extended see-saw models, the mixing can be sizable without contradicting the constraints from neutrino masses. Thus, tests of the unitarity of this matrix are also tests of the nature of the underlying mass generation mechanism.

\subsubsection{Flavor symmetries}
\label{WG1:SubSec:PMNS-Theory:FlavorSymmetries}

Unless a flavor symmetry or some other constraining structure is imposed, the mixing angles and CP-violating phase(s) in the PMNS matrix are arbitrary parameters, similarly to their CKM analogues. However, the measured values of the mixing angles for both the PMNS and CKM matrices do encourage speculations about a deeper flavor structure, which possibly could eventually help solve the long-standing mystery of quark-lepton family replication.

The CKM matrix is famously not very different from the unit matrix, with the largest mixing angle (the Cabibbo angle $\theta_c$) being about $0.23$ and the others one to two orders of magnitude smaller. The PMNS matrix pattern of $\theta_{12}$ and $\theta_{23}$ being large while $\theta_{13}$ is small (but not dissimilar from the Cabibbo angle) presents a contrasting conundrum. A common approach to analysing possible flavor symmetries is to postulate a simple, dominant form for these matrices that is readily associated with a symmetry, and then to introduce deviations to bring the eventual forms into line with the measurements. The unit matrix is one sensible starting point for the CKM matrix. The PMNS matrix, on the other hand, invites several different possibilities for the dominant pattern, which often are special cases of the form
\begin{equation}
    \left( \begin{array}{ccc}
    c_{12} & s_{12} & 0 \\ -s_{12}/\sqrt{2} & c_{12}/\sqrt{2} & -1/\sqrt{2} \\ -s_{12}/\sqrt{2} & c_{12}/\sqrt{2} & 1/\sqrt{2}
    \end{array} \right),
\end{equation}
which has $\theta_{12}$ as a parameter, $\theta_{23}$ set to the maximal value of $\pi/4$ and $\theta_{13}$ equal to zero. While this general pattern was conceived before $\theta_{13}$ was measured to be nonzero, it remains a justifiable zeroth-order ansatz for the PMNS matrix, with finite $\theta_{13}$ and deviations from $\pi/4$ for $\theta_{23}$ ascribed to higher-order corrrections. Commonly considered special cases are (a) \emph{tribimaximal mixing}~\cite{Harrison:2002er} which has $\sin\theta_{12} = 1/\sqrt{3}$, (b) \emph{bimaximal mixing}~\cite{Barger:1998ta,Fukugita:1998vn} which has $\sin\theta_{12} = 1/\sqrt{2}$, and (c) \emph{golden ratio mixing}~\cite{Datta:2003qg,Kajiyama:2007gx,Rodejohann:2008ir} which has $\cos\theta_{12} = \phi/2$ where $\phi = (1 + \sqrt{5})/2$. After the discovery of a relatively large $\theta_{13}$, dominant patterns in which $\theta_{13}$ is nonzero have been put forward; for recent reviews see \cite{Xing:2019vks,Feruglio:2019ktm}.
It should be noted that the PMNS matrix emerges from the diagonalisation of both the charged lepton and neutrino mass matrices and inherits the flavor structure from both sectors.

These patterns are typically derived from discrete or finite flavor
symmetry groups, which may have their origins as discrete subgroups of
continuous flavor groups such as SO(3) and SU(3) or products thereof,
where the ``$3$'' is mandated by the observed threefold family
replication.
Many different groups have been considered, including $S_4$, $A_4$,
$A_5$, $D_N$, $\Sigma(2 N^2)$, $\Sigma(3 N^3)$, $\Delta(3 N^2)$,
$\Delta(6 N^2)$ as well as the continuous groups
$SU(3)$~\cite{Alonso:2013nca} and $SO(3)$~\cite{King:2005bj}.
Tribimaximal mixing (TBM) has mostly been studied in the context of
the $A_4$ and $S_4$ discrete symmetry groups, though several other
possibilities, including $\Delta(27)$, have also received attention.
Bimaximal mixing can also be derived from $S_4$, while golden ratio
mixing is connected with $A_5$
(see~\cite{King:2013eh,Xing:2019vks,Feruglio:2019ktm} and references
therein).
The underlying mechanism assumes that the leptonic doublets are
charged under a specific flavor symmetry $G_f$.
The latter is subsequently broken in order to explain the
non-degenerate charged lepton masses.
The breaking leads to different structures in the charged lepton and
the neutrino sectors,  which ultimately lead to $U_\mathrm{PMNS}$. 

Due to the reduced number of free parameters, a typical prediction for leptonic flavor models is the correlation between mixing parameters, see e.g.~\cite{King:2002nf} and the review in \cite{King:2013eh}, commonly called sum rules.
They can be typically classified into two main groups:
\begin{itemize}
%
\item
Atmospheric sum rules, i.e.\ $\sin^2 \theta_{23} = 1/2 + \zeta \sin
\theta_{13} \cos \delta$, with $\zeta$ a real parameter given by the
model.
A relevant example is trimaximal mixing, which can be obtained from
TBM pattern using a rotation in the 2-3 or 1-3 plane:
$\sin^2 \theta_{23} = 1/2 - \sqrt{2} \sin \theta_{13} \cos \delta$
and $\sin^2 \theta_{23} = 1/2 + 1/ \sqrt{2} \sin \theta_{13} \cos \delta$,
respectively. 
%
\item
Solar sum rules, i.e.\ $\sin^2 \theta_{12}  = 1/3 + \zeta^\prime \sin^2 \theta_{13} \cos \delta $, with $\zeta^\prime$ a real parameter predicted by the model. They are often present in models in which the leading-order mixing matrix gets corrections from the charged lepton sector.
\end{itemize}
If a sufficient precision can be achieved in measuring the mixing angles and the CP-violating phase $\delta$, present and/or future oscillation experiments can test these relations and would be able to provide useful insight on the origin of the observed leptonic flavor structure; see e.g.\ \cite{Ballett:2013wya}.


An interesting class of flavor symmetries are those that non-trivially combine transformations between families with CP transformations, the obvious motivation being to constrain the CP violating phases in the PMNS matrix, especially the Majorana phases. A generalized CP symmetry~\cite{Grimus:1995zi,Feruglio:2012cw,Holthausen:2012dk,Chen:2014tpa} is introduced, which combines charge conjugation and parity and acts in a non-trivial manner on the flavor indices. This symmetry is then combined with a given flavor symmetry. Typically, predictions for the CPV phases, including the Majorana ones, are obtained, leading to testable signatures in neutrino oscillation and neutrinoless double beta decay experiments. A large number of special cases have been analysed in the literature, with useful summaries provided in the reviews of Refs.\cite{Coloma:2018ioo,Xing:2019vks,Feruglio:2019ktm}.

A more recent development~\cite{Feruglio:2017spp} has been the idea of using the non-linearly realized flavor symmetries known as \emph{modular symmetries}, a structure that has its origins in supersymmetry and string theory. In standard flavor symmetry theories, fields transform according to representations of the group, but parameters such as Yukawa coupling constants, while constrained by the symmetries, do not transform. Modular symmetries are extended mathematical structures under which the coupling constants are functions of a chiral superfield $\tau$ called the \emph{modulus}. Requiring modular invariance leads to the coupling constants having to transform in a certain way, thus greatly constraining the form of the theory. This paradigm is able to constrain the neutrino masses in addition to the PMNS parameters~\cite{Xing:2019vks,Feruglio:2019ktm}.

The relationship, if any, between lepton and quark mixing is a very
important issue.
Obviously, any comprehensive theory of flavor has to deal with both
the lepton and the quark sectors.
Grand unified theories, where quarks and leptons reside in the same
irreducible representations of the gauge group, provide strong
theoretical motivation for considering all fermions in an encompassing
flavor scenario.
Some efforts have been made to fit quarks together with leptons in
discrete flavor symmetry schemes (see Sec.~2B of
\cite{Feruglio:2019ktm} for a review).
Grand unification can provide some justification for numerical
relationships between PMNS and CKM parameters such as $\theta_{13}
\sim \theta_c/\sqrt{2}$ and the quark-lepton complementarity relation
$\theta_{12} + \theta_c \sim \pi/4$~\cite{Minakata:2004xt}. 

\subsubsection{CP violation}
\label{WG1:SubSec:PMNS-Theory:CPV}

The PMNS matrix has up to three CP-violating phases. The Dirac phase is the analogue of the CKM CP-violating phase and it can be measured in neutrino oscillation experiments. If neutrinos are Majorana particles, then there are two other phases. They cancel out of oscillation probabilities, but affect other observables such as the neutrinoless double-beta-decay rate. For seesaw models that feature additional, usually very massive, neutral fermions, there will in general be additional CP-violating phases affecting the decays of the heavy neutral fermions into the charged leptons and $W$-bosons or Higgs bosons. The last of these effects is important for leptogenesis driven by out-of-equilibrium heavy neutral lepton decays above the electroweak phase transition~\cite{Fukugita:1986hr}.

Leptogenesis has received great attention because it can naturally take place in see-saw models~\cite{Minkowski:1977sc,GellMann:1980vs,Yanagida:1979as,Glashow:1979nm,Mohapatra:1979ia} and has been shown to be able to explain the observed baryon asymmetry of the Universe. It can be implemented in different ways, depending on the underlying neutrino mass model. In the simplest case of type I see-saw models, it readily satisfies the three Sakharov conditions:
(i) lepton number is violated by the heavy Majorana masses; (ii) several CP-violating phases can be present in the Yukawa coupling between heavy neutrinos and the Higgs; (iii) the departure from equilibrium is guaranteed by the expanding Universe. At very high temperatures, the heavy Majorana neutrinos are in thermal equilibrium with the rest of the plasma due to their Yukawa interactions and decouple after the temperature drops below their mass. In the presence of CP-violation, their decays generate a lepton asymmetry which is converted into a baryon asymmetry by sphaleron processes.


The current experimental preference for a nonzero Dirac phase is an encouraging sign for the existence of new sources of CP violation in nature, as is required for all theories of baryogenesis. The connection with leptogenesis is a very important one, as it could, in principle at least, shed light on the nature of leptonic CP-violation. Unless special flavor structures are imposed, all of these phases are free parameters, whose origin is as much of a mystery as are the fermion masses and lepton and quark mixing angles. Most models of neutrino masses contain a larger number of parameters than those measurable, and in particular more CP-violating phases. Consequently, in a completely model-independent way it is not possible to draw a direct link between the value of $\delta$ and the baryon asymmetry. However, models which aim to explain the values of neutrino masses and of the mixing structure we observe have a reduced number of parameters and can present a direct connection between the two.

It is possible to make some more general statements in specific neutrino mass models. In the widely studied case of the type I see-saw at scales below $10^{12}$~GeV, it can be shown that the $\delta$ phase can be the origin of the observed baryon asymmetry~\cite{Pascoli:2006ie,Pascoli:2006ci,Anisimov:2007mw,Moffat:2018smo}, and it is also possible in extended see-saw models~\cite{Dolan:2018qpy}. This statement is a highly non-trivial since its CP-violating effects are suppressed by the small $\theta_{13}$. This would represent the terrestrial discovery of a parameter that is essential for very early-universe cosmology. Alternatively, if the Dirac phase, depending on its value, could be proven to be inadequate, then that would point to the existence of additional phases, which could well have a leptonic origin.
One can conclude that, generically, the observation of lepton number violation (e.g.\ neutrinoless double beta decay) and of CP violation in long-baseline neutrino oscillation experiments and/or possibly neutrinoless double beta decay would provide circumstantial evidence (even if not a proof) in favor of leptogenesis as the origin of the baryon asymmetry of the Universe.


\subsubsection{Unitarity of the PMNS matrix}
\label{WG1:SubSec:PMNS-Theory:Unitarity}

There will be departures from unitarity for the PMNS matrix when it is a $3 \times 3$ submatrix of a larger unitary matrix that includes additional neutrino or neutrino-like species such as light sterile neutrinos and heavy neutral leptons. This is the case for the type I and III~\cite{Foot:1988aq} seesaw models, and variations such as the inverse and linear~ seesaw models. Barring special flavor structures, one expects the deviations from unitarity to scale as powers of the ratio of the electroweak scale to the large new physics scale, so low-scale seesaw scenarios such as the inverse and linear seesaw models typically provide the largest deviations.

Such deviations affect a raft of precision electroweak and flavor
observables including the $W$-mass, the weak mixing angle, $Z$-decays,
tests of flavor universality, and many others.
A systematic study of such processes that includes evaluation of the
upper bounds on unitarity-violating deviations for each element of the 
PMNS matrix is presented in~\cite{Fernandez-Martinez:2016lgt}.
The upper bounds were obtained by relating the actual mixing matrix
$N$ (as defined through charged-current interactions between charged
leptons and neutrinos) to an exactly unitary matrix $U_\text{PMNS}$
via a Hermitian matrix $\eta$ such that $N = (1 - \eta)U_\text{PMNS}$. 
These results show that deviations up to the $2-7\%$ level are
permitted by current data, depending on the matrix element.
The $\eta_{\tau\tau}$ parameter is the least constrained, with
$\eta_{\mu \mu}$ the most constrained. 


==> WG5/WG5_Summary.tex <==
\subsection{Technologies: Summary}
WR: Probably we can skip this summary. 

==> table.tex <==
%%%%%%%%%%%%%%%%%%%%%% Start table

\begin{table}[t]
\resizebox{\textwidth}{!}{%
    \centering
    \begin{tabular}{lll}\hline\hline
        %
{\bfseries Decay type}    & {\bfseries Project} & {\bfseries Staged goals and projected timelines} \\
\hline
$\beta^-$-decay of \textsuperscript{3}H\textsubscript{2}    &    KATRIN    & First 2 science runs (2019), $m_\beta < 0.8$~eV (90\% C.L.) \cite{Aker:2021gma}\\[0.2ex]
    &        & Data-taking for $0.2$~eV sensitivity ($2019- 2024$)\\[0.2ex]
    &       & R\&D on differential read-out and novel source concepts\\[0.2ex]
    &        & Detector upgrade for keV-sterile $\nu$ search ($>$~2025)\\
\midrule
IC of \textsuperscript{83m}Kr    &    Project 8    & Phase I: demonstration of CRES technique ($2014 - 2016$)  \cite{Asner:2014cwa}\\[0.2ex]
 %& &($2014 - 2016$) \cite{Asner:2014cwa}\\[0.2ex]
$\beta^-$-decay of \textsuperscript{3}H\textsubscript{2}    &        & Phase II: tritium demonstrator ($2015-2020$)\\[0.2ex]
$\beta^-$-decay of \textsuperscript{3}H\textsubscript{2}    &          & Phase III: {\small large-volume CRES demonstrator,  atomic source develop.} \\
& & (R\&D ongoing,  starting 2023 for  $3-5$~eV sensitivity)\\[0.2ex]
%& & sensitivity)\\[0.2ex]
$\beta^-$-decay of \textsuperscript{3}H                                &          & Phase IV: atomic source \\
& & (R\&D ongoing,  starting 2024 for  $40$~meV sensitivity)\\
\midrule
$\nu_e$ capture on \textsuperscript{3}H    & PTOLEMY & R\&D stage, target $m_\beta$ sensitivity $<100$~meV*\\
\midrule
EC of \textsuperscript{163}Ho        & ECHo        & ECHo-1k: Medium-sized array ($\sim$ 100 detectors) \\
&     & First science run (2018), $m_\beta < 150$~eV (95\% C.L.) \cite{Velte:2019jvx}\\
&   & Data-taking for $10 - 20$~eV sensitivity ($2019 - 2020$)\\ [0.2ex]
&     & ECHo-100k: Large array ($\sim$ 12000 detectors)\\ 
&    & Production phase, starting 2021 for $1 - 2$~eV sensitivity \\
\midrule
EC of \textsuperscript{163}Ho        & HOLMES    & Short-term ($2020 - 2021$): Medium-sized array ($\sim$100 channels)\\[0.2ex] 
& & for $10 - 20$~eV sensitivity \\[0.2ex]
& & Medium-term ($2021 - 2023$): Increase number of deployed  \\
& &  arrays ($\sim$ 1000 channels) for $1 - 2$~eV sensitivity \\
\hline\hline
%
\end{tabular}}
\normalsize 
\caption{Overview of current and upcoming experimental approaches in direct kinematic mass measurements using $\beta^-$-decay of molecular and atomic tritium or electron capture in \textsuperscript{163}Ho. Most experiments are taking a phased approach towards improving sensitivity on the neutrino mass. --- *) The PTOLEMY project is intended to become a tritium-based observatory for cosmic relic neutrinos. Its potential to probe neutrino masses is currently being investigated.
    \label{tab:kinematical_exp} }
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% End Table


